Who Is the Strongest Enemy? Towards Optimal and Efficient Evasion Attacks in Deep RL

Evaluating the worst-case performance of a reinforcement learning (RL) agent under the strongest/optimal adversarial perturbations on state observations (within some constraints) is crucial for understanding the robustness of RL agents. However, finding the optimal adversary is challenging, in terms of both whether we can find the optimal attack and how efficiently we can find it. Existing works on adversarial RL either use heuristics-based methods that may not find the strongest adversary, or directly train an RL-based adversary by treating the agent as a part of the environment, which can find the optimal adversary but may become intractable in a large state space. This paper introduces a novel attacking method to find the optimal attacks through collaboration between a designed function named "actor" and an RL-based learner named "director". The actor crafts state perturbations for a given policy perturbation direction, and the director learns to propose the best policy perturbation directions. Our proposed algorithm, PA-AD, is theoretically optimal and significantly more efficient than prior RL-based works in environments with large state spaces. Empirical results show that our proposed PA-AD universally outperforms state-of-the-art attacking methods in various Atari and MuJoCo environments. By applying PA-AD to adversarial training, we achieve state-of-the-art empirical robustness in multiple tasks under strong adversaries. The codebase is released at https://github.com/umd-huang-lab/paad_adv_rl.

==> 3.5_optimal_old.tex <==
%!TEX root = 0_neurips2021_evasionrl_main.tex

\section{Understanding the Optimal State Adversary via Policy Perturbations}
\label{sec:optimal}

In this section, we establish the theory of the optimal adversary for a fixed victim policy $\pi$ by analyzing the connection among the state space, the policy space and the value space, as visualized and summarized by Figure~\ref{fig:diagram}.
% we propose a way to characterize the optimality of evasion attack algorithms. 

\begin{wrapfigure}{r}{0.4\textwidth}
\vspace{-0.5em}
  \centering
  \includegraphics[width=0.4\textwidth]{\fighome/equivalence.pdf}
  \caption{\small{Equivalence between evasion attacks and policy perturbation.}}
  \label{fig:equiv}
\vspace{-1.5em}
\end{wrapfigure}

\subsection{Evasion Attacks Are Perturbations of Policies}
% \yc{our contribution. benefit. figure}
% \textbf{Evasion Attacks Are Perturbations of Policies.} 
% We point out that evasion attacks, no matter on states or actions, are essentially equivalent to perturbing the agent's policy $\pi$ into anther policy $\advpi\in\Pi$. 
Although existing literature usually consider state attacks and action attacks separately, we point out that evasion attacks, no matter applied to states or actions, are essentially equivalent to perturbing the agent's policy $\pi$ into anther policy $\advpi\in\Pi$. 
For instance, as shown in Figure~\ref{fig:equiv}, if the adversary $h$ alters state $s$ into state $\tilde{s}$, then the victim selects an action $\tilde{a}$ based on distribution $\pi(\cdot|\tilde{s})$, the policy on the perturbed state $\tilde{s}$. This is equivalent to directly perturbing $\pi(\cdot|s)$ to $\advpi(\cdot|s):=\pi(\cdot|\tilde{s})$. (See Appendix~\ref{app:relation} for more detailed analysis including action adversaries.)
% Therefore, the perturbation in the policy space is the result, while the perturbation in the state/action space is the cause~\fh{this sentence should be polished, it is a little misleading and ambiguous. Maybe something like, perturbations in either state space or action space will ultimately perturb the policy deployed.}.
% Note that for notation simplicity, the definitions of this paper are based on state adversaries, and Appendix~\todo{app} provides discussions about action adversaries.
In this paper, we characterize attacks from the perspective of policy perturbations caused by an admissible state adversary. 
% therefore it is crucial to characterize the admissible policy perturbations corresponding to the admissible state adversary, under some budget constraint. 
In Definition~\ref{def:pbset}, we formally characterize the admissible policy perturbations as a \pbsetlarge(\pbsetshort) generated by all admissible state adversaries $\adv\in\advset$. 
% Due to the budget constraint, the policy is only perturbed within a subset of the whole policy space $\Pi$. More precisely, the policies generated by all admissible adversaries form a subset of $\Pi$ containing the clean policy $\pi$ as defined in Definition~\ref{def:pbset}.
% The concept of policy perturbation provides a tool to understand evasion attacks in RL in a more unified way. 
% In this paper, as in most literature, we mainly focus on the adversary that applies state perturbations, i.e., the adversary perturbs a state $s\in\states$ to $\tilde{s} \in \ball_{\epsilon}(s)$, where $\ball_\epsilon$ denotes an $\ell_p$ norm ball with radius $\epsilon$. 
% But note that a simplified version of our method can be applied to action perturbations.

% Formally, we denote the evasion adversary by a deterministic function $\adv: \Pi \to \Pi$ which perturbs the victim policy $\pi$ into policy $\adv(\pi)$. 
% For notation simplicity, define $\advpi := \adv(\pi)$. 
% For a fixed victim policy $\pi$, the goal of the adversary is to find an optimal $\adv^*$ such that $V^{\advpi^*}$ is minimized over all \textit{admissible} adversaries.
% An evasion adversary $\adv$ is said to be admissible if the policy perturbation can be achieved with the attack constraint, i.e., $\forall s\in \states, \exists \tilde{s} \in \ball_{\epsilon}(s) \text{ s.t } \advpi(s) = \pi(\tilde{s})$. We denote the set of all admissible adversaries by $\advset$.

\begin{definition}[\textbf{\pbsetlarge(\pbsetshort)}]
\label{def:pbset}
  For an MDP $\mdp$, a fixed policy $\pi$, we define the \pbsetname(\pbsetshort) w.r.t. $\pi$, denoted as $\pbset$,  as the set of policies that are perturbed from $\pi$ by all admissible adversaries, i.e., $\pbset := \{ \tilde{\pi}\in\Pi: \exists \sadv \in \sadvset \text{ s.t } \tilde{\pi}(s) = \pi(\sadv(s)), \forall s \}$.
\end{definition}

\textbf{Remarks.} (1) \pbsetshort is a Cartesian product of $|\states|$ subsets of simplices.
(2) For a continuous mapping $\pi$ (e.g., a neural network), \pbsetshort is connected and compact as proven in Appendix~\ref{app:notations}.
% Since the perturbations in the state space are within an $\ell_p$ norm ball, and the policy network is a continuous mapping, we~\fh{formally prove} that a \pbsetshort is connected and compact~\fh{as in Appendix xx Theorem xx.}\yc{The proof is just this sentence}.
 
\textbf{The Merits of Considering Policy Perturbations.}
(1) The search space could be reduced. In many environments, the state space $\states$ is continuous, and much larger than the action space $\actions$. But the original space of all adversary functions is of cardinality $|\states|^{|\states|}$ since both the domain and image spaces are $\states$, which is computationally prohibitive. 
In contrast, if we map the perturbation to the policy space, the cardinality of all policy perturbations is of cardinality $|\states|^{|\prob(\actions)|}$ (for a stochastic victim $\pi$), or $|\states|^{|\actions|}$ (for a deterministic victim $\pi_D$).
(2)
% There is a more certain relationship between policies and values~\cite{dadashi2019the}~\fh{this is unclear, what do you mean?}. 
By converting the adversarial perturbations from the state/action space into the policy space, we can better understand the optimality of adversaries, through analyzing the optimality of the perturbed policy.
% Theorem~\ref{thm:opt_adv} relates the optimal adversary and the values of the perturbed policy. And Theorem~\ref{thm:polytope} characterizes the shape of the value space of policies in \pbsetshort.  
% We let $\advpi$ denote the policy perturbed from $\pi$ by adversary adversary $\sadv \in \sadvset$. (The superscript $^{(\states)}$ is omitted when there is no ambiguity.)
(3) Policy perturbation unifies state and action attacks. Existing works usually consider state attacks and action attacks differently. However, an ideally robust model should be robust to any kind of attacks. Policy perturbation captures the essence of evasion attacks, making it possible to consider state and action attacks simultaneously.

% \yc{1. definition and comparison 2. existence and characterization (is it easy to optimize over the PPS by their values?) 3. topological interpretation}

\begin{figure*}[!t]
 \vspace{-2em}
  \begin{center}
   \includegraphics[width=0.8\textwidth]{\fighome/diagram_new.pdf}
  %\vspace{-3pt}
  \caption[center]{\small{The process of evasion attacking. A state adversary $\adv$ perturbs $s$ into $\adv(s)$ in the state space; hence, the victim's policy $\pi$ is perturbed into $\advpi$; as a result, the expected total rewards the victim can gain from $s$ becomes $V^{\advpi}$ instead of $V^\pi$.
  The attacker's goal is to minimize the value in the value space by perturbing the state observation (input to the policy network) in the state space.
  Finding the optimal adversary is an RL problem.
  A prior work~\cite{zhang2021robust}(we will refer as \saname) directly uses an RL agent to learn the best state perturbation, which works for MDPs with small state space, but suffer from high complexity in larger MDPs.
  In this paper, we dive deeper into the process of evasion attacks, and find that policy perturbations are the bridge connecting state perturbations and value perturbations. 
  By decoupling the attack problem into an RL part (finding the policy with the lowest value) and a non-RL part (perturbing the state to force the policy network to have some specific outputs), our proposed attack method called \ours achieve both optimal and efficient attacks.
  }}
  \label{fig:diagram}
  \end{center}
  \vspace{-1.5em}
\end{figure*}

\subsection{The Relation between State Adversaries and Policy Perturbations}
\label{sec:existence}

The goal of the attacker is to find a state adversary that minimizes the victim's expected total return in the environment. Therefore, we first formulate the definition of an optimal state adversary as below.

\begin{definition}[\textbf{Optimal State Adversary}]
	For an MDP $\mdp$, a fixed policy $\pi$, and an admissible adversary set $\advset$, an optimal state adversary satisfies $\adv^* \in \mathrm{argmin}_{\adv \in \advset} V^{\advpi}_{\mdp} (s), \forall s\in\states$.~ Recall that $\advpi$ is the perturbed policy $\pi_h(\cdot|s)=\pi(\cdot|\tilde{s})$.
\end{definition}

It has been shown by~\cite{zhang2020robust} that learning the optimal state adversary is equivalent to learning the optimal policy in another MDP, and there exists an optimal state adversary for a fixed victim policy $\pi$.
However, as Figure~\ref{fig:diagram} shows~\fh{it seems that this is the only place that we mentioned Figure~\ref{fig:diagram}: we need a better description of the figure using words; where should we put this figure? }, what a state adversary essentially does is to perturb the policy $\pi$ to $\advpi$ which has lower values. Therefore, the optimality of the adversary can be characterized by the corresponding policy perturbation. Proposition~\ref{prop:opt_adv} shows that there exists a policy in the \pbsetshort $\pbset$ such that the value is minimized, and such a policy is corresponding to the optimal state adversary.

\begin{proposition}[\textbf{Existence of the Optimal Policy Perturbation}]
\label{prop:opt_adv}
	For an MDP $\mdp$, a fixed policy $\pi$, and an admissible adversary set $\advset$, there exists an optimal perturbed policy $\advpiopt \in \mathrm{argmin}_{\advpi \in \pbset} V^{\advpi}_{\mdp} (s), \forall s\in\states$. 
	Moreover, for any optimally perturbed policy $\advpiopt$, there exists at least one optimal state adversary that perturb $\pi$ into $\advpiopt$.
\end{proposition}
\textbf{Remarks.} 
(1) The proof in Appendix~\ref{app:existence} shows that learning the optimally perturbed policy is equivalent to learning the optimal policy in another MDP. 
(2) There might exist more than one optimally perturbed policies, and more than one optimal state adversaries. 
(3) The perturbed policy generated by any optimal state adversary is optimal. And any state adversary that can generate an optimally perturbed policy is optimal. Thus, Proposition~\ref{prop:opt_adv} shows the equivalence between the optimal perturbation in the state space (discussed in~\cite{zhang2020robust}) and the optimal perturbation in the policy space. 
(4) Optimal policy perturbations are also connected with optimal action-space perturbations.

% Theorem~\ref{thm:opt_adv} defines an optimal adversary as the adversary that makes the agent get the lowest possible total reward among all admissible adversaries.
% The proof of Theorem~\ref{thm:opt_adv} is deferred to Appendix~\todo{app:existence}, which justifies that learning the optimal adversary is equivalent to learning the optimal policy in another MDP.
% (3) \cite{zhang2020robust} has shown a similar result on state adversaries, while our formulation is based on policy perturbations, which include both state and action adversaries.


\subsection{The Relation between Policy Perturbations and the Value Functions}
Section~\ref{sec:existence} establishes the relation between state perturbations and policy perturbations: an optimal policy perturbation is generated by an optimal state adversary, and vice versa. 
So, one can first find the optimal policy perturbation, then compute the corresponding optimal state adversary.
How to identify the optimal policy perturbation?
Recall that an ``optimal'' adversary should reduce the policy value the most.
Therefore, in this section we study how the value $V^\pi$ of policy $\pi$ changes when $\pi$ varies in the \pbsetshort $\pbset$.
In summary, we first show that policies in the \pbsetshort $\pbset$ have bounded and structured values, then we prove that the ``boundary'' of the \pbsetshort always contains the optimal policy perturbation.
% Although we have established that the optimal policy perturbations and optimal state perturbations are closely related~\fh{not only closely related right? be more specific? map to each other?}, optimizing the policy perturbation over an unknown \pbsetshort ~\fh{I feel this abbreviation could make the reading not very smooth, could we change the name, maybe admissible policy perturbations? and not use the abbreviation?} is still difficult. 
% But fortunately~\fh{remove such wording in technical writing}, we find that \pbsetshort has some nice properties~\fh{what nice property?}, due to the fact that \pbsetshort is a connected and compact subset of the whole policy space $\Pi$~\fh{this sentence needs to be polished.}.
% \fh{I think you can summarize this subsection here. (1) lay out the difficulty of learning optimal policy perturbation. (2) summarize our result, say something like: We will first prove that admissible/bounded state perturbations lead to bounded policy perturbations, which then lead to bounded value perturbations. We then show that the optimal policy perturbation lies on the boundary of the admissible policy perturbation set. (I am using a wrong terminology here for PPS, try deciding on a terminology).}

\textbf{The Values of \pbsetshort Are Structured.}
The following theorem describes the ``shape'' of the value functions corresponding by all possible policy perturbations given by admissible adversaries.
Roughly speaking, bounded state perturbations lead to bounded policy perturbations, which then result in bounded value perturbations. 
\begin{theorem}[\textbf{Policy Perturbation Polytope}]
\label{thm:polytope}
	For a finite MDP $\mdp$, consider a policy $\pi$ and a \pbsetshort $\pbset$. The space of values (a subspace of $\mathbb{R}^{|\states|}$) of all policies in $\pbset$, denoted by $\mathcal{V}_{\pbset}$, is a (possibly non-convex) polytope.
\end{theorem}

Theorem~\ref{thm:polytope} is an extension of the result in~\cite{dadashi2019the}, which shows that the values of the whole policy space $\mathcal{V}$ is a polytope.
As shown in Figure~\ref{fig:diagram} right, both $\mathcal{V}$ and $\mathcal{V}_{\pbset}$ are polytopes. 
And Figure~\ref{fig:example} in Appendix~\ref{app:example} shows the polytopes generated from a real MDP example.
See Appendix~\ref{app:polytope} for more details and proofs of Theorem~\ref{thm:polytope}. 



\textbf{The Boundary of \pbsetshort Contains An Optimal Policy Perturbation.}
Recall that the optimal state adversary can be found by finding the optimally perturbed policy in the \pbsetshort $\pbset$. However, the budget constraint is defined in the state space, and it is difficult to directly compute the \pbsetshort. Then, is there a way to find the optimally perturbed policy without knowing the exact $\pbset$?
Theorem~\ref{thm:boundary} suggests that one can always find an optimal adversary on the ``outermost boundary'' of the \pbsetshort. Therefore, an attacker can push the victim policy as far as possible using all his budget without missing the optimality. 
\begin{theorem}
  \label{thm:boundary}
  For an MDP $\mdp$, a fixed policy $\pi$, and a admissible adversary set $\advset$, define the \textbf{outermost boundary} of the \pbsetname $\pbset$ w.r.t $\pi$ as 
  \setlength\abovedisplayskip{2pt}
  \setlength\belowdisplayskip{2pt}
  \begin{equation*}
  \omboundary \pbset := \{ \pi^\prime \in \pbset: \forall s \in \states, \nexists \theta>0 \text{ s.t. } \pi^\prime(\cdot|s) + \theta(\pi^\prime(\cdot|s)-\pi(\cdot|s)) \in \pbset \}
  \end{equation*}
  Then there exists a policy $\tilde{\pi} \in \omboundary \pbset$, such that $\tilde{\pi}$ is the optimally perturbed policy w.r.t. $\pi$ over all policies in $\pbset$.
  % the adversary $\adv(\pi)=\tilde{\pi}$ is the optimal adversary for $\pi$ in $\mdp$.
\end{theorem}
Note that the outermost boundary of $\pbset$~\fh{give an english name(terminology) for this $\pbset$} is w.r.t.~\fh{corresponding to?} an anchor policy $\pi$ ~\fh{Why does it have to a point? Why it is not a line? Then the line would correspond to a set of policies? Also, here is $\pi$ any policy or the victim's policy? It seems that we are mixing the notation throughout the paper a little bit. Could you fix that?}.
Intuitively, one can imagine that for any state $s$, there are infinitely many rays emitted from $\pi(s)$ to all possible directions in simplex $\Pi_s$~\fh{What do you mean here?}. And a policy $\pi^\prime$ is in $\omboundary$ iff for every $s\in\states$, $\pi^\prime(\cdot|s)$ is the farthest point that $\pi(\cdot|s)$ can reach by following the corresponding ray in direction $\pi^\prime(\cdot|s)-\pi(\cdot|s)$~\fh{it is not very clear, could you clarify? What is the major message of this theorem?}.
The proof of Theorem~\ref{thm:boundary} is in Appendix~\ref{app:boundary}. 
Inspired by these theoretical results, we propose our attack algorithm in Section~\ref{sec:algo}, that efficiently searches for the optimally perturbed policy using the state-space constraint.
% Based on this result, if an adversary is able to perturb a policy within a neighborhood, then he can directly push the policy as much as possible using all his budget without missing the optimality. 



% In Section~\ref{sec:algo}, we further characterize the relations among perturbations in state, policy and value space, and then propose our algorithm based on theoretical insights. 

% \subsection{Optimality of Evasion Attack Formulations}
% \label{sec:opt_formulation}

% There are many existing evasion attack methods in RL~\cite{huang2017adversarial,pattanaik2018robust,zhang2020robust}, while it is not yet well-understood how strong these attacks are in general, and whether they can find the optimal adversaries for any problem. 
% Intuitively, an attack method is not optimal if the optimal solution to its objective, if exists, is not the optimal adversary for the given victim policy.
% Therefore, we define the concept of optimal formulation for evasion attacks in RL in Definition~\ref{def:optimal}, which characterizes the optimality of the formulation of a problem.  
% \begin{definition}[Optimal Formulation for Evasion Attacks]
% \label{def:optimal}
% 	An attacking algorithm $\mathrm{Algo}$ is said to have an optimal formulation iff for any MDP $\mdp$, policy $\pi$ and admissible adversary set $\advset$, the set of optimal solutions to its objective, $\advset^{\mathrm{Algo}}$, is a subset of optimal adversaries, i.e., $\advset^{\mathrm{Algo}} \subseteq \advset^*:=\{\adv^*| \adv^* \in \mathrm{argmin}_{\adv \in \advset} V^{\advpi}_{\mdp} (s), \forall s\in\states\}$.
% \end{definition}
% % As discussed in Section~\ref{sec:existence}, finding the optimal adversary is an RL problem. 
% Many heuristic methods, although are empirically effective and efficient, do not meet the requirements of optimal formulation, as proven inn Appendix~\todo{heuristics}.
% In the scenario where finding the worst-case performance of an agent is crucial, heuristic methods may not be strong enough.
% A recent work~\cite{zhang2021robust} uses an RL formulation, which is theoretically an optimal formulation, but not efficient when the state space is large. In Section~\ref{sec:algo}, we will elaborate the efficiency problem in~\cite{zhang2021robust} and propose our solutions.
% \yc{simply describe some heuristic attacks, and point out that they are not optimal (emphasis the importance of optimality)}







==> 4_greedy.tex <==
%!TEX root = 0_neurips2021_evasionrl_main.tex

\section{Characterizing Optimality of Heuristic Attacks}
\label{sec:greedy}

There are many existing methods of finding adversarial state perturbations for a fixed RL policy, most of which are solving some optimization problems defined by heuristics. 
Although these methods are empirically shown to be effective in many environments, it is not clear how strong these adversaries are in general. 
% A natural question to ask is: 
% \textit{can we minimize the expected total reward of the agent with these heuristic adversaries?}
In this section, we carefully summarize and categorize existing heuristic attack methods into 4 types, and then characterize their optimality in theory.

\textbf{\textit{TYPE \RNum{1}} - Minimize The Best (\minbest).}
A common idea of evasion attacks in supervised learning is to reduce the probability that the learner selects the ``correct answer''~\cite{ian2015explaining}. 
Prior works~\cite{huang2017adversarial,kos2017delving,ezgi2020nesterov} apply a similar idea to craft adversarial attacks in RL, where the objective is to minimize the probability of selecting the ``best'' action, i.e.,
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\begin{equation}
	\label{eq:minbest}
	\tag{\RNum{1}}
	\advminbest \in \mathrm{argmin}_{\adv \in \advset} \advpi(a^+|s), \forall s\in\states
\end{equation}
where $a^+$ is the ``best'' action to select at state $s$. \cite{huang2017adversarial} define $a^+$ as $\mathrm{argmax}_{a\in\actions} Q^\pi(s,a)$ for DQN, or $\mathrm{argmax}_{a\in\actions} \pi(a|s)$ for TRPO and A3C with a stochastic $\pi$. Since the agent's policy $\pi$ is usually well-trained in the original MDP, $a^+$ can be viewed as (approximately) the action taken by an optimal deterministic policy $\pi^*(s)$.
% Note that different from supervised learning where the correct answers are known as labels, in RL, we do not know which action is the best. Instead, one can only learn a Q function for a specific policy, $Q^\pi(s,a)$. Then for any state $s$, $a^+ := \mathrm{argmax}_{a\in\actions} Q^\pi(s,a)$ is the approximated ``best'' action.
% However, different from supervised learning where the correct answer is known and unique, in RL, we do not know which action is ``correct'', and whether or not an action is good also depends on future decisions. Therefore, some previous works propose to maximize the difference between the perturbed policy and a ``good policy'', and prevent the agent from selecting the good policy's action. The objective can be abstracted as

% where $\pi^+$ is the ``good'' policy defined by specific algorithms. For example, the MAD attack proposed by~\cite{zhang2020robust} uses the agent's current policy $\pi$ as $\pi^+$, and maximizes the distance between the perturbed policy and the original policy.
% Prior to this method, the idea of~\cite{huang2017adversarial} is also to maximize the difference between the perturbed policy and a ``best'' policy $\pi^+$, which is a deterministic version of the agent's well-trained policy, i.e., $\pi^+ = \mathrm{argmax}_{a\in\actions} \pi(a|s), \forall s\in\states$.

\textbf{\textit{TYPE \RNum{2}} - Maximize The Worst (\maxworst).}
\cite{pattanaik2018robust} point out that only preventing the agent from selecting the best action does not necessarily result in a low total reward. Instead, \cite{pattanaik2018robust} propose another objective function which maximizes the probability of selecting the worst action, i.e.,
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\begin{equation}
	\label{eq:maxworst}
	\tag{\RNum{2}}
	\advmaxworst \in \mathrm{argmax}_{\adv \in \advset} \advpi(a^-|s), \forall s\in\states
\end{equation}
where $a^-$ refers to the ``worst'' action at state $s$. 
\cite{pattanaik2018robust} defines the ``worst'' action as the actions with the lowest Q value, which could be ambiguous, since the Q function is policy-dependent. 
If a worst policy $\pi^- \in \mathrm{argmin}_\pi V^\pi(s), \forall s \in \states$ is available, one can use $a^- = \mathrm{argmin} Q^{\pi^-}(s,a)$. However, in practice, the attacker usually only has access to the agent's current policy $\pi$, so he can also choose $a^- = \mathrm{argmin} Q^{\pi}(s,a)$. 
Note that these two selections are different, as the agent's policy $\pi$ is usually far away from the worst policy.
We discuss the optimality of both selections in Appendix~\todo{app:heuristic}.
% To make the definition more rigorous, we define $a^-$ in two ways:
% (1) $a^-_{\pi^-} := \mathrm{argmin} Q^{\pi^-}(s,a), \forall s\in\states$, where $\pi^-$ is the worst deterministic policy on $\mdp$.
% (2) $a^- := \mathrm{argmin} Q^{\pi}(s,a), \forall s\in\states$, where 
% However, different from the best action $a^+$ which can be approximated by a well-trained policy, the worst policy is usually not known to the attacker. 
% There are two potential solutions to this challenge: (1) if the attacker has access to the environment, he may first search for a policy $\pi^-$ with the lowest value, then use $\pi^-$ to generate $a^-$;
% (2) as \cite{pattanaik2018robust}, the attacker 
% \yc{There are different ways to understand the meaning of the ``worst'' action. (1) The actions taken by the deterministic worst policy. (2) The actions that have the lowest Q value evaluated on the current policy.}

\textbf{\textit{TYPE \RNum{3}} - Minimize Q Value (\minq).}
Another idea of attacking~\cite{pattanaik2018robust,zhang2020robust} is to craft perturbations such that the agent selects actions with minimized Q values at every step, i.e.,
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\begin{equation}
	\label{eq:minq}
	\tag{\RNum{3}}
	\advminq \in \mathrm{argmin}_{\adv \in \advset} \sum\nolimits_{a\in\actions} \advpi(a|s) \hat{Q}^{\pi}(s, a), \forall s\in\states
\end{equation}
where $\hat{Q}$ is the approximated Q function of the agent's original policy. For example, \cite{pattanaik2018robust} directly uses the agent's Q network (of policy $\pi$), while \cite{zhang2020robust} learns a more stable Q network for the agent's policy $\pi$. 
Note that in practice, this type of attack is usually applied to deterministic agents (e.g., DQN, DDPG, etc), then the objective becomes $\mathrm{argmin}_{\adv \in \advset} \hat{Q}^{\pi}(s, \advpi(s)), \forall s\in\states$~\cite{pattanaik2018robust,zhang2020robust,oikarinen2020robust}.

\textbf{\textit{TYPE \RNum{4}} - Maximize Difference (\maxdiff).}
The MAD attack proposed by~\cite{zhang2020robust} is to maximize the distance between the perturbed policy $\advpi$ and the clean policy $\pi$, i.e.,
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\begin{equation}
	\label{eq:maxdiff}
	\tag{\RNum{4}}
	\advmaxd \in \mathrm{argmax}_{\adv \in \advset} \mathrm{KL}[ \advpi(s) || \pi(s) ], \forall s\in\states
\end{equation}
where $\mathrm{KL}$ denotes the KL-divergence between two distributions.  
This type of attack is inspired by the fact that if two policies select actions with similar action distributions on all the states, then the value of the two policies is also small (see Theorem 5 in~\cite{zhang2020robust}).


These heuristic methods are often able to reduce the rewards of the agent in practice. However, it is not yet understood whether these objectives are optimal in general cases, which is important in terms of understanding the worst-case performance of an agent. 
In general, an attack method is formulated in an optimal way if the exact solutions to the objective function are also optimal adversaries. Otherwise, even if we solve the optimization problem perfectly, the corresponding attack is still not the strongest. 
We describe the optimal formulation of attacks in Definition~\ref{def:optimal}.  
\begin{definition}[Optimal Formulation for Evasion Attacks]
\label{def:optimal}
	An attacking algorithm is said to have optimal formulation if for any MDP $\mdp$, policy $\pi$ and admissible adversary set $\advset$, the set of optimal solutions to its objective, $\advset^{\mathrm{Algo}}$, is a subset of optimal adversaries, i.e., $\advset^{\mathrm{Algo}} \subseteq \advset^*:=\{\adv^*| \adv^* \in \mathrm{argmin}_{\adv \in \advset} V^{\advpi}_{\mdp} (s), \forall s\in\states\}$.
\end{definition}

Based on the above definition, Theorem~\ref{thm:heuristic} shows that none of the above heuristic formulations is optimal, and the optimal solutions to objectives~\eqref{eq:minbest}, \eqref{eq:maxworst}, \eqref{eq:minq} and \eqref{eq:maxdiff}, denoted as $\advsetminbest, \advsetmaxworst, \advsetminq$ and $\advsetmaxd$ respectively, may not contain the optimal adversary.
\begin{theorem}[\textbf{Optimality of Heuristic Attacks}]
\label{thm:heuristic}
	Suppose $\pbset\subsetneqq\Pi$, then \minbest, \maxworst, \minq and \maxdiff are not optimal formulations. 
	Moreover, there exist an MDP $\mdp$ and an agent policy $\pi$, such that $\advsetminbest$ (similarly, $\advsetmaxworst, \advsetminq$ and $\advsetmaxd$) does not contain an optimal adversary $\adv^*$, i.e., $\advsetminbest \cap \advset^* = \emptyset$.
\end{theorem}
We prove Theorem~\ref{thm:heuristic} by constructing counter examples where the minimizers or maximizers to Problem~\eqref{eq:minbest}, \eqref{eq:maxworst}, \eqref{eq:minq} and \eqref{eq:maxdiff} have much higher values than another admissible adversary $\adv \in \advset$. 
Thus the optimal solutions to the above 4 types of attacks are not necessarily optimal adversaries, and optimal adversaries may not be the optimal solutions to these heuristic objectives.
See Appendix~\todo{app:heuristic} for detailed proofs.

Why is it hard for heuristic methods to find the optimal adversary? As Theorem~\ref{thm:opt_adv} suggests, learning the optimal adversary is an RL problem. 
For solving an RL problem, one needs to interact with the environment and iteratively search for the best policy, unless the environment dynamics are known. 
Therefore, single-step optimizations based on only the agent's current policy are not enough for finding the optimal adversary.





==> 5_algo_old.tex <==
%!TEX root = 0_iclr2022_evasionrl_main.tex

\section{\ours: Optimal and Efficient Evasion Attack}
\label{sec:algo}
% \yc{(1) inefficiency (2) how to propose directions}
% \yc{1. inefficiency of SARL and our disentanglement
% 2.  our algorithm high-level description (how to propose directions) 
% and theoretical justifications (optimality and efficiency)
% 3. implementation details
% }
% \subsection{Motivation}
% \label{sec:algo_motiv}
% Section~\ref{sec:optimal} re-formulates the optimal attacking problem in RL through the lens of the optimal policy adversary. 
In this section, we first formally define the optimality of an attack algorithm and discuss some existing attack methods.
% summarize some existing evasion RL methods with a focus on their optimality and efficiency.
Then, we introduce our algorithm, \textit{\oursfull (\ours)} that has an optimal formulation and is efficient to use.
% efficiently finds the optimal adversary for a fixed victim policy.
%  prior evasion RL methods, including heuristic methods that are efficient but may not be optimal, and RL-based methods that learn the optimal adversary but may be inefficient.
% Then, 
% and propose our algorithm, \textit{\oursfull (\ours)}, that efficiently finds the optimal adversary for a fixed victim policy.

Although many evasion attack methods have been proposed~\citep{huang2017adversarial,pattanaik2018robust,zhang2020robust}, it is not yet well-understood how to characterize the strength of an attack algorithm.
Therefore, we propose to formulate the optimality of an attack algorithm, which answers the question ``whether the attack objective finds the strongest adversary''.
% define \textit{optimal formulation} for evasion attacks in RL in Definition~\ref{def:optimal} as below.
% , which characterizes the optimality of the formulation of a problem.  
\begin{definition}[Optimal Formulation for Evasion Attacks]
\label{def:optimal}
  An attacking algorithm $\mathsf{Algo}$ is said to have an optimal formulation iff for any MDP $\mdp$, policy $\pi$ and admissible adversary set $\advset$ under attacking budget $\epsilon$, the set of optimal solutions to its objective, $\advset^{\mathsf{Algo}}$, is a subset of optimal adversaries, i.e., $\advset^{\mathsf{Algo}} \subseteq \advset^*:=\{\adv^*| \adv^* \in \mathrm{argmin}_{\adv \in \advset} V^{\advpi}_{\mdp} (s), \forall s\in\states\}$.
\end{definition}
% \textbf{Remarks.} 
% (1) Recall that $\advset$ contains adversaries with a certain attack budget $\epsilon$. 
% % An optimally formulated algorithm works for any given $\epsilon\geq 0$.
% (2) Intuitively, an attack method is optimally formulated if any optimal solution to its objective is an optimal adversary for the given victim $\pi$ and budget $\epsilon\geq 0$.

% Section~\ref{sec:optimal} shows that finding the optimal adversary is an RL problem.
% Therefore, many heuristic methods, although are empirically effective and efficient, do not meet the requirements of optimal formulation, as proven in Appendix~\ref{app:optimal_heuristic}.
% Therefore, in the scenarios where finding the worst-case performance of an agent is crucial, heuristic methods may not be strong enough.
\begin{figure*}[!b]
 \vspace{-0.5em}
  \begin{center}
   \includegraphics[width=\textwidth]{\fighome/pa-ad-compare.pdf}
  \vspace{-1.5em}
  \caption[center]{\small{An overview of \ours compared with a heuristic attacker and an end-to-end RL attacker. 
  % A heuristic attacker directly perturbs each state based on heuristics (e.g., minimize the probability that the agent chooses its original action). 
  Heuristic attacks are efficient, but may not find the optimal adversary as they do not learn from the environment dynamics. 
  An end-to-end RL attacker directly learns a policy to generate state perturbations, but is inefficient in large-state-space environments. 
  In contrast, our \textbf{\ours} solves the attack problem with a combination of an RL-based director and a non-RL actor, so that \ours achieves both optimality and efficiency.
  % ~\fh{I like the figure, great job!}
  }}
  \label{fig:paad}
  \end{center}
  \vspace{-1.5em}
\end{figure*}

Intuitively, an attack method is optimally formulated if any optimal solution to its objective is an optimal adversary for the given victim $\pi$ and budget $\epsilon\geq 0$.
Many heuristic-based attacks, although are empirically effective and efficient, do not meet the requirements of optimal formulation.
In Appendix~\ref{app:optimal_heuristic}, we categorize existing heuristic attack methods into four types, and theoretically prove that they may not find the strongest adversary in some cases.
% there exist scenarios where these heuristic methods may not find the strongest adversary.
A recent paper~\citep{zhang2021robust} proposes to learn the optimal state adversary using RL methods, which we will refer to as \textit{\saname} in our paper for simplicity. \saname can be viewed as an ``end-to-end'' RL attacker, as it directly learns the optimal state adversary such that the value of the victim policy is minimized. 
The formulation of \saname satisfies Definition~\ref{def:optimal} and thus is optimal.
% The adversary of \saname takes the original state $s$ as the input, and outputs a constrained state perturbation $\tilde{s}\in\ball_\epsilon(s)$ as the action. 
% Whenever the victim agent receives a reward $r$, the adversary gets a reward $-r$. 
% In this way, if the adversary maximizes its own cumulative reward, then the agent's cumulative reward is minimized.
However, \saname learns an MDP whose state space and action space are both the same as the original state space. 
% which can be high-dimensional in practice (e.g. Atari games).
% In Section~\ref{sec:exp}, \saname works similarly to a random attacker, as the adversary is learning an MDP with both the state space and the action space being image spaces.
If the original state space is high-dimensional (e.g. images), learning a good policy in the adversary's MDP may become computationally intractable, as empirically shown in Section~\ref{sec:exp}.
% then the state space and action space of the new MDP are both large, making it prohibitive to learn a good policy, as empirically shown in Section~\ref{sec:exp}. 
% However, if the state space is high-dimensional (e.g. images), then the state space and action space of the new MDP are both large, making it prohibitive to learn a good policy, as empirically shown in Section~\ref{sec:exp_atari}. 

Can we address the optimal attacking problem in an efficient manner?
As shown in Figure~\ref{fig:diagram}, a state perturbation leads to a policy perturbation, and then the policy perturbation results in a value perturbation; only the latter process depends on the environment dynamics and requires learning, while the former process is similar to evasion attacks in a supervised learning problem and does not require learning.
Therefore, we propose a novel algorithm, \textit{\oursfull (\ours)}, that has optimal formulation and is generally more efficient than an end-to-end RL adversary.
\ours decouples the whole attacking process into two simpler components: policy perturbation and state perturbation, solved by a ``director'' and an ``actor'', respectively. The director learns the optimal policy perturbing direction with RL methods, while the actor crafts adversarial states at every step such that the victim policy is perturbed towards the given direction.
In Appendix~\ref{app:compare_sa}, we provide a comprehensive comparison between \ours and \saname from multiple aspects.


% \subsection{Our Algorithm: \oursfull (\ours)}
% \label{sec:algo_overview}
% \textbf{Our method \ours: cooperation between a director and an actor.}

% The former solves the RL part and the latter deals with the non-RL part. 
% An overview of our algorithm compared with \saname and heuristic attackers is demonstrated in Figure~\ref{fig:paad}. 
% Heuristic attacks~\citep{huang2017adversarial,pattanaik2018robust,zhang2020robust} craft adversarial states at every step separately, without considering the correlations among steps; an end-to-end RL attacker~\citep{zhang2021robust} learns the optimal state perturbations directly using RL methods, although might be not efficient. 
% \ours can be regarded as a novel combination of these two types of attacks: 

% As shown in Figure~\ref{fig:paad} right, the director is learning an RL policy $\nu$, whose observation is the states of the original environment, action is a signal to the actor denoting ``which direction to perturb the victim policy into''.
% And the actor is denoted by a function $g$, which maps the director's action into a perturbed state $\tilde{s}\in\ball_\epsilon(s)$.

Formally, for a general stochastic victim policy $\pi$, our proposed \ours algorithm solves a \textit{Policy Adversary MDP (PAMDP)} defined in Definition~\ref{def:adv_mdp}. An actor denoted by $g$ is embedded in the dynamics of PAMDP, and a director searches for an optimal policy $\nu^*$ in the PAMDP.
% director learns an RL policy $\nu$ in a \textit{Policy Adversary MDP (PAMDP)} defined in Definition~\ref{def:adv_mdp}, while the actor denoted by $g$ is embedded in the dynamics of PAMDP, mapping a target direction and the current state to a perturbed state. Theorem~\ref{thm:optimality} proved in Appendix~\ref{app:optimal} further justifies the optimality of PAMDP.
% The input of $\nu$ is the current state in the original environment, while the output is a signal to the actor denoting ``which direction to perturb the victim policy into''.
% The actor denoted by function $g$ is a part of the MDP dynamics, which maps the director's action and the current state $s$ into a perturbed state $\tilde{s}\in\ball_\epsilon(s)$ and send it to the victim.
% Detailed explanations are provided later.
\begin{definition} [\textbf{Policy Adversary MDP (PAMDP) $\widehat{\mdp}$}]
% \vspace{-0.5em}
\label{def:adv_mdp}
  Given an MDP $\mdp= \langle \states, \actions, \dynamics, \rewards, \gamma \rangle$, a fixed stochastic victim policy $\pi$, a budget $\epsilon \geq 0$, we define a Policy Adversarial MDP $\widehat{\mdp}=\langle \states, \widehat{\actions}, \widehat{\dynamics}, \widehat{\rewards}, \gamma \rangle $,
  % where the state space is $\widehat{\states}=\states$, 
  % \\
  % (1) for a stochastic victim $\pi$:
  where the action space is {\small{$\widehat{\actions}\!=\!\{d\in \!\!{[0,1]}^{|\actions|}, \sum_{i=1}^{|\actions|} d_i = 0 \}$}},
  and $\forall s,s^\prime \in \states, \forall \widehat{a}\in \widehat{\actions}$,
  \setlength\abovedisplayskip{2pt}
  \setlength\belowdisplayskip{2pt}
  {\small{
  \begin{equation*}
  \widehat{\dynamics}(s^\prime|s,\widehat{a})=\sum\nolimits_{a\in \actions} \pi(a|g(\widehat{a},s)) \dynamics(s'|s,a), \quad \widehat{\rewards}(s,\widehat{a}) = - \sum\nolimits_{a\in\actions} \pi(a|g(\widehat{a},s))\rewards(s,a).
  \end{equation*}
  }}
  % $\widehat{\dynamics}(s^\prime|s,\widehat{a})=\sum_{a\in \actions} \pi(a|g(\widehat{a})) \dynamics(s'|s,a), \forall s,s^\prime \in \states$, 
  % and the reward function is
  % $\widehat{\rewards}(s,\widehat{a}) = - \sum_{a\in\actions} \pi(a|g(\widehat{a}))\rewards(s,a)$.
  % \setlength\abovedisplayskip{2pt}
  % \setlength\belowdisplayskip{2pt}
  % \begin{equation*}
  % \widehat{\rewards}(s,\widehat{a}) = 
  % \begin{cases} 
  %   - \sum_{a\in\actions} \pi(a|g(\widehat{a}))\rewards(s,a) & \text{if} \; \norm{g(\widehat{a})} \in \ball_{\epsilon}(s) \\
  %   % \text {and} \;\pi(\cdot |s)+ \widehat{a}\in \Delta(\actions)   \\ 
  %   -\infty & \text{otherwise};
  % \end{cases}
  % \end{equation*} 
  % :\!\widehat{\actions} \times \states\!\!\to\!\states
  The actor function $g$ is defined as 
  \setlength\abovedisplayskip{2pt}
  \setlength\belowdisplayskip{2pt}
  \begin{equation}
  \label{eq:actor}
  \tag{$G$}
    g(\widehat{a},s) = \mathrm{argmax}_{s'\in B_{\epsilon}(s)}\norm{\pi(s')-\pi(s)}
    \text{ subject to }\big(\pi(s')-\pi(s)\big)^T \widehat{a}=\norm{\pi(s')-\pi(s)}\norm{\widehat{a}}.
  \end{equation}
\vspace{-1.5em}
\end{definition}


The input to director policy $\nu$ is the current state $s$ in the original environment, while its output $\widehat{a}$ is a signal to the actor denoting ``which direction to perturb the victim policy into''. 
% (The director's action space {\small{$\widehat{\actions}$}} contains all possible perturbing directions in {\small{$\prob(\actions)$}}.)
% Then, the actor maps the director's action and the current state $s$ into a perturbed state $\tilde{s}\in\ball_\epsilon(s)$ and sends it to the victim.
The actor, once receiving the perturbing direction $\widehat{a}$, will ``push'' the policy as far as possible by perturbing $s$ to $g(\widehat{a},s)\in\ball_\epsilon(s)$, as characterized by the optimization problem~\eqref{eq:actor}.
Therefore, the director and the actor together induce a state adversary: $\adv(s):=g(\nu(s),s), \forall s\in\states$. 
In this way, the policy perturbation resulted by the director and the actor is always in the outermost boundary of $\pbset$ w.r.t. the victim $\pi$, where the optimal policy perturbation can be found according to Theorem~\ref{thm:boundary}.
Therefore, \ours has an optimal formulation as stated in Theorem~\ref{thm:optimality} (proven in Appendix~\ref{app:optimal}).
% Theorem~\ref{thm:optimality} (proven in Appendix~\ref{app:optimal}) shows that the optimal solutions to \ours are optimal adversaries against any victim policy and any budget $\epsilon$, which justifies that \ours has an optimal formulation.
\begin{theorem}[\textbf{Optimality of \ours}]
% \vspace{-1em}
  \label{thm:optimality}
  For any MDP $\mdp$, a fixed victim policy $\pi$, and any attack budget $\epsilon\geq0$, an optimal policy $\nu^*$ in $\widehat{\mdp}$ induces an optimal state adversary against $\pi$ in $\mdp$.
  That is, the formulation of \ours is optimal, i.e., $\advsetours \subseteq \advset^*$.
\vspace{-0.5em}
\end{theorem}

\textbf{Efficiency of \ours} \quad
% Note that \saname uses an RL formulation, which is also theoretically optimal, but not efficient when the state space is large. 
% In contrast, \ours is more efficient due to the advanced design of the MDP.
As commonly known, the sample complexity of solving an RL problem grows with the cardinalities of the state space and the action space. Both \saname and \ours have state space $\states$, the state space of the original MDP. But the action space of \saname is also $\states$, while our \ours has action space $\mathbb{R}^{|\actions|-1}$. % (or $\actions$ for deterministic victim policies).
% \footnote{
%   When the original MDP has a continuous action space (e.g. MuJoCo), the agent usually takes actions deterministically during test time, so the action space of the adversary's MDP is $\widehat{\actions}$.
% }.
In many applications, the state space (e.g. a pixel space) is in a higher dimensional space than $\mathbb{R}^{|\actions|-1}$, then \ours is generally more sample efficient than \saname.%, and can find the optimal state adversary more quickly.
% In the case of deterministic victims, the adversary's MDP has the same size of the original MDP and will not be much harder to learn than the original environment.




% The learning process is: at step $t$, the director observes a state $s_t$, and proposes a policy perturbation $\widehat{a}$, then the actor searches for a state perturbation to meet the policy perturbation, afterwards, the victim receives the perturbed state $\tilde{s}$ and outputs its action $a_t$, finally the environment returns the next state $s_{t+1}$ and reward $r_t$, and the director obtains $- r_t$ as its own reward. 
\textbf{Variants of \ours} \quad
Our \ours can be (1) further simplified for a deterministic victim policy, and (2) extended to environments with continuous action spaces.
For (1), the PAMDP in Definition~\ref{def:adv_mdp} focuses on a general stochastic victim, which samples action $a$ from distribution $\pi(\cdot|s)$ at state $s$.
Attacking a stochastic victim is generally more challenging than attacking a deterministic victim due to the randomness of action sampling. 
% which is often ignored in existing methods. 
% Define $\pi_D$ as a deterministic version of policy $\pi$, i.e., $\pi_D(s) := \mathrm{argmax}_{a\in\actions} \pi(a|s)$.
For a deterministic victim policy, we define a simpler Deterministic Policy Adversary MDP (D-PAMDP) in Appendix~\ref{app:algo_det}, where the action space of the director is the same as the original action space of the victim, i.e., $\actions$. 
In short, in D-PAMDP, the director proposes a target action $\widehat{a}_D \in \actions$, and the actor conducts targeted attacks to let the victim output the target $\widehat{a}_D$.
% , i.e., the actor conducts targeted attack for the current state with $\widehat{a}_D$ as the target action.
For (2), when the action space is continuous, the actor instead minimizes the distance between the policy action and the target action, i.e., $\mathrm{argmax}_{s^\prime\in B_{\epsilon}(s)} \|\pi(s^\prime) - \widehat{a}_D\|$.
\emph{In the deterministic case, Theorem~\ref{thm:optimality} (the optimality of \ours) still holds}, as proven in Appendix~\ref{app:optimal_det}.
Moreover, since the action space of D-PAMDP is $\actions$, smaller than the action space of the stochastic PAMDP, \emph{the efficiency of \ours is further improved in the deterministic case}.
Appendix~\ref{app:algo} provides more details and formal definitions of the aforementioned variants of our method. 
In Section~\ref{sec:exp}, we show experimental results for deterministic victim agents in continuous action spaces. 



\textbf{Implementation Details} \quad
For the deterministic variant of \ours described in Appendix~\ref{app:algo}, the actor's objective~\eqref{eq:actor_det} is simple and can be directly solved to identify the optimal adversary.
In contrast, the actor's objective for a stochastic victim defined in~\eqref{eq:actor} requires solving a more complex optimization problem, which in practice can be relaxed to~\eqref{eq:actor_relax} (a Lagrangian relaxation) to efficiently get an approximation of the optimal adversary.
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\begin{align}
\label{eq:actor_relax}
\tag{$\hat{G}$}
  \mathrm{argmax}_{s^\prime \in B_{\epsilon}(s)} L(s^\prime;\widehat{a}, s) := \norm{{\pi}(\cdot|s^\prime)-\pi(\cdot|s)}  + \lambda \times \mathsf{CosineSim}\big(\pi(\cdot|s^\prime)-\pi(\cdot|s),\: \widehat{a} \big) 
% \label{eq:actor_det_relax}
% \tag{$\hat{G}_D$}
%  &\mathrm{argmax}_{s^\prime \in B_{\epsilon}(s)} L_D(s,\pi) := \mathsf{CrossEntropy}(\pi(s^\prime), \widehat{a}_D)
\end{align}
where $\mathsf{CosineSim}$ refers to the cosine similarity function; the first term measures how far away the policy is perturbed from the victim policy; $\lambda$ is a hyper-parameter controlling the trade-off between the two terms.
Note that the relaxation is only needed for a stochastic victim. In Appendix~\ref{app:discuss}, we discuss the optimality of this relaxation. 
We also evaluate the effects of hyperparameter $\lambda$ in Appendix~\ref{app:exp_hyper}.
% (we set $\lambda$ as 1 in experiments).
% The first term measures the alignment of the actual policy perturbation direction and the proposed perturbation direction, while the second term measures how far away the policy is perturbed; 
% $\beta$ is a hyper-parameter controlling the trade-off between two terms.
% The above implementation, although finds the approximations to the optimal policy, achieves effective and efficient evasion attacks in our experimental results as shown in Section~\ref{sec:exp}.
The procedure of learning the optimal adversary is depicted in Algorithm~\ref{alg:main}, where we simply use the Fast Gradient Sign Method (FGSM)~\citep{ian2015explaining} to approximately solve the actor's objective, although more advanced solvers such as Projected Gradient Decent (PGD) can be applied.
Experiment results in Section~\ref{sec:exp} verify that the above implementation achieves state-of-the-art attack performance.

\vspace{-0.5em}
\input{algo_main}
\vspace{-0.5em}



==> algo_main_det.tex <==
%!TEX root = 0_neurips2021_evasionrl_main.tex

\begin{algorithm}[H]
% \vspace{-1em}
\SetAlgoLined
\textbf{Input:} Initialization of director's policy $\nu$; victim policy $\pi$; budget $\epsilon$; start state $s_0$ %, $\lambda\;(\lambda>0)$
\\
\For{$t=0,1,2,...$}{
	\textit{Director} samples a policy perturbing direction $\widehat{a}_t \sim \nu(\cdot|s_t)$\\
% Compute loss function for actor:\\
% $L(s_t,\delta_t, \tilde{\pi}(\cdot|s_t))=-\:\text{CosineSim}\Big(\pi(\cdot|s_t+\delta_t)-\pi(\cdot|s_t),\: \hat{a}_t \Big)-\alpha \norm{{\pi}(\cdot|s_t+\delta_t)-\pi(\cdot|s_t)}$\\
	% \vspace{-0.2em}
	\textit{Actor} sets $\tilde{s}_t = s_t + \epsilon\cdot\text{sign}(\nabla_{\delta} L_D(s_t+\delta; \widehat{a}_t, s_t ) )$ where 
	$$
	L_D(s^\prime;\widehat{a}, s) := \pi(\widehat{a}|s^\prime) - \mathrm{max_{a\in\actions, a \neq \widehat{a}}} \pi(a|s^\prime)
	$$
	\textit{Victim} takes action $a_t\sim \pi(\cdot|\tilde{s}_t)$, proceeds to {{$s_{t+1}\sim \dynamics(s_{t+1}|s_t, a_t)$}}, receives {{$r_t = \rewards(s_t,a_t)$}}\\
	\textit{Director} saves $(s_t,\widehat{a}_t,-r_t,s_{t+1})$ to its buffer \\	
	\textit{Director} updates its policy $\nu$ using any RL algorithm
}
\caption{\oursfull (\ours) - For Deterministic Victim}
\label{alg:main_det}
\end{algorithm}

==> defs.tex <==
%!TEX root = 0_iclr2021_evasionrl_main.tex


\section{Unifying Evasion Attacks in RL}

In RL, an agent interacts with the environment modeled by a Markov Decision Process (MDP), which is denoted by a tuple $\mdp=\langle \states, \actions, \dynamics, \rewards, \gamma \rangle$, where $\states$ is the state space, $\actions$ is the action space, $\dynamics: \states \times \actions \to \prob(S)$ is the transition function \footnote{$\prob(X)$ denotes the the space of probability measures over $X$}, $\rewards: \states \times \actions \to \mathbb{R}$ is the reward function, and $\gamma \in (0, 1)$ the discount factor. 
At time $t$, the agent observes state $s_t$, takes action $a_t$ and then receives a reward $r_t$. How to take actions is controlled by the \textit{policy} the agent uses, $\pi: \states \to \prob(\actions)$. In this paper we focus on stationary, stochastic policies. In test time, the agent uses a fixed policy $\pi$ such that $a_t \sim \pi(s)$. Denote the whole policy space as $\Pi := \prob(\actions)^{|S|}$. 
% The value of a policy for state $s$ is defined as $V^\pi(s) = \mathbb{E}_{\pi}[\sum_{t=0}^\infty \gamma^t R(s_t,r_t)|s_0=s]$. 
% The general goal of RL is to find a policy that maximizes the corresponding value. According to the classic MDP theory~\cite{puterman2014markov}, there exists a deterministic policy $\pi^*$ that has the highest value for all states, i.e., $V^{\pi^*}(s) = \max_{\pi} V^\pi(s), \forall s$, namely the optimal policy in MDP $\mdp$.

\textbf{State Attacks and Action Attacks.}
Evasion attacks are test-time attacks that influence the actual behaviors of the agent/victim. As in most literature, we study non-targeted evasion attacks in RL, i.e., the goal of the adversary is to reduce the cumulative reward gained by the victim during test time. In general, the adversary can not directly change the environment, but can (1) perturb a state returned by the environment before the victim observes it; (2) perturb an action taken by the victim before the environment receives it. In either case, we assume the amount of perturbation is upper bounded by some constant $\epsilon$, to make the attacks realistic in practice.
% Note that in supervised learning, an evasion adversary usually only perturbs the input data, while in RL, both states (input) and actions (output) may subject to perturbations due to the interactive process.
Formally, we assume the adversary attacks by a deterministic function denoted by $\adv$.
(1) A state adversary $\sadv$ perturbs the state, i.e., $\sadv(s;\pi)=\tilde{s}$, where $\tilde{s} \in \ball_{\epsilon^{(S)}}(s) := \{ s^\prime \in \states: \| s^\prime - s \| \leq \epsilon^{(S)}\}$
(2) An action adversary $\aadv$ perturbs the action, i.e., $\aadv(a;s,\pi)=\tilde{a}$, where $\tilde{a} \in \ball_{\epsilon^{(A)}}(a) := \{ a^\prime \in \actions: \| a^\prime - a \| \leq \epsilon^{(A)}\}$. \cite{tessler2019action} define another type of action perturbation based on a discrete action space and a stochastic adversary, which is discussed in our Appendix XX.
% if the action space is discrete, then the constraint is $\| \tilde{\pi}(\cdot|s) - \pi(\cdot|s) \| \leq \epsilon^{(A)}$, where $ \tilde{\pi}(a^\prime|s) = \mathrm{Pr}[\aadv(a;s,\pi)=a^\prime | s], \forall a^\prime \in \actions$.


\textbf{The Essence: Policy Perturbation.}
State attacks and action attacks, although differ by definitions and manifestations, are both essentially perturbing the victim's policy $\pi$ to a perturbed policy $\tilde{\pi}$. For state adversary $\sadv$



\textbf{What Are the Advantages of Studying Policy Perturbations?}
\yc{Why do we care policy perturbation? The relationship between policy and value is easier to characterize -- polytope theory}












==> fig_polytope.tex <==
%!TEX root = 0_iclr2021_evasionrl_main.tex

\vspace*{-0.5em}
\begin{figure}[!htbp]
\centering
	\begin{subfigure}[t]{0.24\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{\fighome/line.png}
	\caption{}
	\label{sfig:line}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.24\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{\fighome/perturb_one.png}
	\caption{}
	\label{sfig:perturb}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.5\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{\fighome/compare.pdf}
	\caption{}
	\label{sfig:compare}
	\end{subfigure}
	\vspace*{-1em}
	\caption{\small{\textbf{(a)} The values of all policies in $\Pi$ form a polytope (blue region); the values of all policies agreeing on all but one state form a line segment (yellow line). \textbf{(b)} Perturb a given $\pi$ to $\tilde{\pi}$ within a connected and compact subset of policies $\ball(\pi) \subseteq \Pi$, the values of perturbed policies also form a polytope (green region), or a line segment if only perturb $\pi$ on one state. \textbf{(c)} Comparison of the optimality of different adversaries. The mapping from policy space (left) to the value space (right). Our method finds the policy perturbation that achieves the lowest reward among all perturbations.}}
	\label{fig:example}
\end{figure}
\vspace*{-0.5em}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> table_attack_robust.tex <==
%!TEX root = 0_neurips2021_evasionrl_main.tex

\begin{table}[!htbp]
\centering
\vspace{-1em}
\caption{\small{Average episode rewards $\pm$ standard deviation of robustly-trained models under different evasion attack methods.}}
\label{tbl:robust}
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{5pt}
% \begin{tabular}{c *{4}{c} p{0.5\tabcolsep} *{6}{c}}
\begin{tabular}{*{9}{c}}
\toprule
% \multirow{2}{*}{\textbf{Environment}} & \multicolumn{4}{c}{\textbf{Properties}} &&  \multicolumn{6}{c}{\textbf{Attack Methods}} \\
%  \cmidrule(r){2-5} \cmidrule(l){7-12}
\textbf{Environment} & \textbf{Model} & \textbf{\specialcell{Natural \\Reward}} & $\boldsymbol{\epsilon}$ & \textbf{Random} & \textbf{\specialcell{\maxdiff\\ \cite{zhang2020robust}}} & \textbf{\specialcell{RS\\ \cite{zhang2020robust}}} & \textbf{\specialcell{\saname\\ \cite{zhang2021robust}}} & \textbf{\specialcell{\ours \\(ours)}} \\
\midrule
\multirow{2}{*}{\textbf{Hopper}} & SA-PPO &   \\
\cmidrule(l){2-9}
& SA-RL-PPO & \\
\midrule
\multirow{2}{*}{\textbf{Walker}} & SA-PPO &   \\
\cmidrule(l){2-9}
& SA-RL-PPO & \\
\midrule
\multirow{2}{*}{\textbf{HalfCheetah}} & SA-PPO &   \\
\cmidrule(l){2-9}
& SA-RL-PPO & \\
\midrule
\multirow{2}{*}{\textbf{Ant}} & SA-PPO &   \\
\cmidrule(l){2-9}
& SA-RL-PPO & \\
\bottomrule
\end{tabular}
}
% \vspace{-1em}
\vspace{-1em}
\end{table}






==> table_dqn_ppo.tex <==
%!TEX root = 0_iclr2021_evasionrl_main.tex

\begin{table}[!htbp]
\vspace{-1em}
\resizebox{1\textwidth}{!}{%
\setlength{\tabcolsep}{1.75pt}
\begin{tabular}{c *{2}{c} p{0.5\tabcolsep} *{6}{c}}
\toprule
\multirow{2}{*}{\textbf{Victim}} & \multicolumn{2}{c}{\textbf{Properties}} &&  \multicolumn{6}{c}{\textbf{Attack Methods}} \\
 \cmidrule(r){2-3} \cmidrule(l){5-10}
 & \textbf{Clean Reward} & $\epsilon$ && \textbf{Random} & \textbf{\specialcell{MinBest\\\citeauthor{huang2017adversarial}} } & \textbf{\specialcell{MaxWorst\\\citeauthor{pattanaik2018robust}}} & \textbf{\specialcell{MAD\\\citeauthor{zhang2020robust}}} & \textbf{\specialcell{\saname\\\citeauthor{zhang2021robust}}} & \textbf{\ours (ours)} \\
 \midrule
 \textbf{DQN} & $96.09 \pm4.04$ & 0.001 && $94.94\pm 4.35$	 & $55.12\pm 11.45$ & $68.93\pm 10.67$ & $82.02\pm 8.98$ & $94.90\pm 4.36$ & $\boldsymbol{23.64\pm 16.72}$\\
  \midrule
 \textbf{DQN} & $96.09 \pm4.04$ & 0.0005 && $94.48\pm 5.30$	 & $84.45\pm 7.40$ & $93.97\pm 4.21$ & $90.25 \pm 6.08$ & $95.33 \pm 4.82$ & $\boldsymbol{82.511\pm 8.62}$\\
 \midrule
\textbf{PPO} & $87.70 \pm 5.89$ & 0.003 && $87.58\pm 6.0$	& $25.23\pm 10.56$ & $7.87\pm 6.67$ & $53.6\pm 11.83$	& $87.73\pm5.28$ &	$\boldsymbol{-1.62\pm 6.39}$\\
 \midrule
\textbf{PPO} & $87.70 \pm 5.89$ & 0.005 && $87.53\pm 5.16$ & $45.34\pm 12.44$ & $\boldsymbol{23.8\pm 9.87}$ & $69.22\pm 11.71$ & $87.62\pm 5.04$ & $26.69\pm 12.06$ \\
\bottomrule
\bottomrule
\end{tabular}
}
\vspace{-1em}
\caption{\small{Comparison of evasion attack methods against PPO and DQN victim on BoxingNoFrameskip-v4. The results are averaged over 1000 episodes.}}
\label{tbl:dqn_ppo}
\vspace{-1em}
\end{table}



==> theory.tex <==
%!TEX root = 0_iclr2021_evasionrl_main.tex

% \section{Optimality of Evasion Attacks in RL}

\section{Problem Setup: RL and Evasion Attacks}
\label{sec:setup}

\textbf{Preliminaries and Notations.}
In RL, an agent interacts with the environment modeled by a Markov Decision Process (MDP), which is denoted by a tuple $\mdp=\langle \states, \actions, \dynamics, \rewards, \gamma \rangle$, where $\states$ is the state space, $\actions$ is the action space, $\dynamics: \states \times \actions \to \prob(S)$ is the transition function \footnote{$\prob(X)$ denotes the the space of probability measures on $X$}, $\rewards: \states \times \actions \to \mathbb{R}$ is the reward function, and $\gamma \in (0, 1)$ is the discount factor. 
The agent takes actions based on a \textit{policy} $\pi: \states \to \prob(\actions)$.  
% In test time, the agent uses a fixed policy $\pi$ such that $a_t \sim \pi(s_t)$ at timestep $t$. 
The value of a policy is defined as $V^\pi(s)=\mathbb{E}[\sum_{t=0}^\infty \gamma^t r_t | s_0=s]$.
We denote the whole policy space as $\Pi := \prob(\actions)^{|S|}$.
% The \textit{value} of a policy can be denoted as a $|\states|$-dim vector $\val^\pi$, with the $i$-th element being the value of $\pi$ starting from $s_i$, i.e., $\val^{\pi}[i]=V^\pi(s_i)=\mathbb{E}[\sum_{t=0}^\infty \gamma^t r_t | s_0=s_i]$.
% At timestep $t$, the agent observes state $s_t$, takes action $a_t$ and then receives a reward $r_t$. How to take actions is controlled by the \textit{policy} the agent uses, $\pi: \states \to \prob(\actions)$. In this paper we focus on stationary, stochastic policies. In test time, the agent uses a fixed policy $\pi$ such that $a_t \sim \pi(s_t)$. Denote the whole policy space as $\Pi := \prob(\actions)^{|S|}$. In this section, we assume $\states$ and $\actions$ are discrete and finite for simplicity, but the algorithm and the experiments in later sections include continuous $\states$ and $\actions$.
% \textit{Evasion attacks} are test-time attacks that influence the actual behaviors of a well-trained agent/victim. 
% As in most literature, we study non-targeted evasion attacks in RL, i.e., the goal of the adversary is to reduce the cumulative reward gained by the victim during test time. 
% Different from evasion attacks in supervised learning where only the input data may be altered, a test-time adversary in RL may have two options: (1) perturb a state returned by the environment before the victim observes it, as in~\cite{huang2017adversarial,pattanaik2018robust,zhang2020robust}; (2) perturb an action taken by the victim before the environment receives it, as in~\cite{tessler2019action,tan2020robustifying}. In either case, perturbation radius is upper bounded by some small constant $\epsilon$ to avoid being detected. Note that we do not consider the scenario where the adversary changes the environment, since it is less universal in practice.
As is common in previous works, we assume the adversary does not have access to the environment, but has access to the victim's parameters (white-box attacking). We mainly focus on state attacks in this work, while our method can be used to conduct action attacks. We use notation $\tilde{s}$ to denote a state perturbed from $s$. 
The perturbation radius is upper bounded by the budget $\epsilon$, i.e., $\tilde{s}\in \ball_{\epsilon}(s)$, where $\ball$ denotes a norm ball.

\textbf{Evasion attacks are perturbations of policies.} Although existing literature usually consider state attacks and action attacks separately, we note that attacking states and attacking actions are essentially equivalent to manipulating the victim's policy. For instance, if the adversary alters state $s$ into state $\tilde{s}$, then the victim selects an action based on distribution $\pi(\cdot|\tilde{s})$, the policy on the perturbed state $\tilde{s}$. This is equivalent to directly perturbing $\pi(\cdot|s)$ to $\tilde{\pi}(\cdot|s):=\pi(\cdot|\tilde{s})$. (See Appendix xx for analysis of action attacks). Throughout this paper, we use $\adv: \Pi \to \Pi$ to denote an evasion attacker, and $\adv(\pi)=\tilde{\pi}$ suggests that $\adv$ perturbs $\pi$ into $\tilde{\pi}$.


\section{Characterizing Optimality of Evasion Attacks} 

% Existing evasion RL works have defined the adversary in different ways, while many of them are following non-optimal formulations. 
% In this section, we provide a formal definition of optimal adversary in RL, and compare existing attack methods via analysis and visualization.

\textbf{What Is An Optimal Adversary?}
% As discussed in Section~\ref{sec:setup}, an evasion adversary forces the victim to execute a perturbed policy $\tilde{\pi}$ instead of the clean policy $\pi$. 
% Finding the optimal adversary is essential to understanding the robustness of machine learning models. 
% And the first step toward finding the optimal adversary is to define what an ``optimal'' adversary is. 
In supervised learning, the optimal adversary is the one that can reduce the victim's predicting accuracy the most. 
However, in RL, the performance of the victim is usually measured by the long-term reward. 
Therefore, the optimal adversary should \textit{reduce the expected cumulative reward as much as possible}, i.e., the value of perturbed policy $V^{\tilde{\pi}}$ is minimized over all feasible $\tilde{\pi}$'s.
(the set of policies that the adversary can perturb $\pi$ into under all constraints). 
\begin{definition}[Optimal Adversary]
\label{def:opt_adv}
	For a given MDP $\mdp$ and a fixed policy $\pi$ on $\mdp$, the optimal adversary $h^*$ satisfies 
	% \begin{equation}
	$h^* = \mathrm{argmin}_{h} V^{\tilde{\pi}}_{\mdp} (s), \forall s\in\states$, where $\pi$ is perturbed into $\tilde{\pi}$ by $h$.
	% \end{equation}
\end{definition}

\textbf{Remarks.} (1) For a fixed policy, there always exists an optimal (and deterministic) adversary, as proved in Appendix XX. Learning the optimal adversary is equivalent to learning the optimal policy in an RL problem.
(2) \citet{zhang2020robust} have shown a similar result on state adversaries, while our formulation is based on policy perturbations.

% Now the optimal attack problem becomes: the adversary perturbs the victim's policy such that the perturbed policy has low value in the original MDP. 
% Hence, it is important to understand the relationship between \textit{``perturbation in the policy space''} and \textit{``perturbation in the value function space''}.
\textbf{How Does ``Policy Perturbation'' Relate to ``Value Perturbation''?}
Now the optimal attack problems becomes to perturb a policy $\pi$ in $\tilde{\pi}^*$ such that $V^{\tilde{\pi}^*}(s) \geq V^{\tilde{\pi}}(s)$ for all state $s$.
A recent paper~\citep{dadashi2019the} presents some topological properties of the relationship between policy space and the value function space.
In summary, in a finite-state MDP, the value (vectors) produced by all policies form a (possibly non-convex) polytope. The value (vectors) generated by policies that agree on all but one state $s$ form a line segment.
% , which can be bracketed by two policies that are deterministic on $s$.
For example, Figure~\ref{sfig:line} shows the value vectors generated by 5M random policies for an MDP with $|\states|=2, |\actions|=3$ (see Appendix xx for the description of the MDP), where we can see the values form a polytope (blue). 
% Moreover, we fix $\pi(s_2)$ and randomly vary $\pi(s_1)$, the resulted values form a line (yellow). The 
In this work, we extend the results of \cite{dadashi2019the} to a subset of the whole policy space, summarized in Theorem~\ref{thm:perturbation} and visualized in Figure~\ref{sfig:perturb}. See Appendix XX for technical details. 

\begin{theorem}[Policy Perturbation Polytope]
\label{thm:perturbation}
	Given a policy $\pi$, let $\ball(\pi) \subseteq \Pi$ be a connected and compact subset of policies containing $\pi$, then the values of $\ball(\pi)$ form a polytope containing $V^\pi$. If policies in $\ball(\pi)$ only differ at one state, then the values of $\ball(\pi)$ lie on a line segment. Moreover, there always exists a policy on the boundary of $\ball(\pi)$ that achieves the lowest value for all states (corresponds to the optimal adversary).
\end{theorem}

\input{fig_polytope}

% \yc{We have an interesting observation that the objectives of most previous evasion attacks are partially following this theoretical framework, although being myopic and non-optimal in the long run. Appendix XXX provides detailed explanations. (Move to appendix?)}

\textbf{Most Previous Evasion Attacks Are Myopic and Non-optimal.}
The objectives of most previous evasion attacks, although partially following the above theoretical framework, are myopic and non-optimal. 
For instance, below are the objectives of 3 well-known evasion RL methods, we will show that the policy perturbations that satisfy these objectives are not optimal adversaries, even in the simplest setting where only the policy at one state is perturbed.
% Below we list some prior evasion attack methods and analyze their optimality .
\begin{itemize}[noitemsep,leftmargin=*,topsep=-1pt]
\item \textbf{[MinBest~\citep{huang2017adversarial}]}: minimizes the probability that the victim chooses the ``best action'' (action with highest Q value) at every state;
% i.e., $\max_{\tilde{\pi}} \mathsf{CrossEntropy}( \tilde{\pi}(s), \pi^{\mathrm{best}}(s))$, where $\pi^{\mathrm{best}}(s)$ chooses the best action at state $s$ with probability 1.
% \begin{equation}
% \max_{\tilde{\pi}} \mathsf{CE}( \tilde{\pi}(s), \pi^{\mathrm{best}}(s)), 
% \text{ where } \pi^{\mathrm{best}}(a|s) := 
% \{ \begin{array}{ll}
%       1 & a = \mathrm{argmax}_a Q^\pi(s,a) \\
%       0 & \text{otherwise}
%     \end{array} 
% \end{equation}
\item \textbf{[MaxWorst~\citep{pattanaik2018robust}]}: maximizes the probability that the victim chooses the ``worst action'' (action with lowest Q value) at every state;
% i.e., $\min_{\tilde{\pi}} \mathsf{CrossEntropy}( \tilde{\pi}(s), \pi^{\mathrm{worst}}(s))$, where $\pi^{\mathrm{worst}}(s)$ chooses the worst action at state $s$ with probability 1.
% \begin{equation}
% \min_{\tilde{\pi}} \mathsf{CE}( \tilde{\pi}(s), \pi^{\mathrm{worst}}(s)), 
% \text{ where } \pi^{\mathrm{worst}}(a|s) := 
% \{ \begin{array}{ll}
%       1 & a = \mathrm{argmin}_a Q^\pi(s,a) \\
%       0 & \text{otherwise}
%     \end{array} 
% \end{equation}
\item \textbf{[KL~\citep{zhang2020robust}]}: maximizes the KL-divergence between the clean policy $\pi$ and the perturbed policy $\tilde{\pi}$.
% i.e., $\max_{\tilde{\pi}} \mathsf{KL}( \tilde{\pi}(s), \pi(s))$
% \begin{equation}
% \max_{\tilde{\pi}} \mathsf{KL}( \tilde{\pi}(s), \pi(s)), 
% \end{equation}
\end{itemize}

% In the above formulations, $\mathsf{CE}$ denotes the cross-entropy loss, and $\mathsf{KL}$ stands for the KL divergence. 
% For illustration simplicity, we only present the objectives of each method, without considering the constraints. 
% $\tilde{\pi}$ refer to the perturbed policy as discussed in Section~\ref{sec:setup}, while in the original papers, $\max_{\tilde{\pi}}$ is achieved through $\max_{\tilde{s}} \pi(\tilde{s})$.

We implemented and tested these three methods in the example 2-state MDP used in Figure~\ref{sfig:line}, and visualize the results in Figure~\ref{sfig:compare}. 
For simplicity, assume the adversaries can perturb only perturb $\pi$ at $s_1$ within a $\ell_2$ norm ball of radius 0.2. As shown in Figure~\ref{sfig:compare}(left), all possible $\tilde{\pi}(s_1)$'s form a disk in the policy simplex, and executing above methods leads to 3 different policies on this disk.
As our theoretical results suggest, the resulted value vectors lie on a line segment shown in Figure~\ref{sfig:compare} (right), where one can see that MinBest, MaxWorst and KL all fail to find the optimal adversary (the policy with lowest value). On the contrary, our method, which will be given in Section~\ref{sec:algo}, finds the optimal adversary that achieves the lowest reward over all policy perturbations.
% , so that even the exact solutions to the objectives are found, they are still not guaranteed to be the optimal adversaries

% And there is another common glitch of [MinBest] and [MaxWorst]: the $Q$ function ...






